Learning Hamiltonian Dynamics with Reproducing Kernel Hilbert Spaces and Random Features

A method for learning Hamiltonian dynamics from a limited and noisy dataset is proposed. The method learns a Hamiltonian vector field on a reproducing kernel Hilbert space (RKHS) of inherently Hamiltonian vector fields, and in particular, odd Hamiltonian vector fields. This is done with a symplectic kernel, and it is shown how the kernel can be modified to an odd symplectic kernel to impose the odd symmetry. A random feature approximation is developed for the proposed odd kernel to reduce the problem size. The performance of the method is validated in simulations for three Hamiltonian systems. It is demonstrated that the use of an odd symplectic kernel improves prediction accuracy and data efficiency, and that the learned vector fields are Hamiltonian and exhibit the imposed odd symmetry characteristics.

==> sections/3_old.tex <==

As the number of trajectories and samples in the training set increases, the size of the learning problem \eqref{eq:vector_valued_regular_least_squares} increases, increasing the training time for the model coefficients. Furthermore, the inference time of the learned model \eqref{eq:vector_valued_regular_least_squares_f_equation} increases. To limit training and inference time random features are used to approximate the kernel functions associated with functions in an RKHS \cite{Singh2021}.

Let the matrix-valued kernel function ${\boldK : \Rn \times \Rn \rightarrow \Rmm}$ be approximated by the matrix-valued feature map ${\boldPsi : \Rn \rightarrow \Rdm}$ \cite{Sindhwani2018} as follows
\begin{equation}
    \boldK(\boldx,\boldy) \approx \boldPsi(\boldx)^{\T} \boldPsi(\boldy)
\end{equation}
Then the function value of the vector field in \eqref{eq:vector_valued_regular_least_squares_f_equation} can be parameterized as
\begin{equation}\label{eq:rkhf_f_using_rff}
    \boldf(\boldx) = \sum_{i=1}^{N} \boldK(\boldx,\boldx_i) \bolda_i \approx \sum_{i=1}^{N} \boldPsi(\boldx)^{\T} \boldPsi(\boldx_i) \boldc_i = \boldPsi(\boldx)^{\T} \boldalpha
\end{equation}
where ${\boldc_i \in \mathbb{R}^m}$, and the new model coefficients are
\begin{equation}
    \boldalpha = \sum_{i=1}^{N} \boldPsi(\boldx_i) \boldc_i \in \Rd
\end{equation}
This makes ${\boldf(\boldx)}$ a linear combination of ${d}$ random feature functions, instead of ${N}$ kernel functions. The number of random features ${d}$ is chosen by balancing the quality of the approximation and the computational time of the function. Using \eqref{eq_inner_prod_func_in_rkhs} and \eqref{eq:rkhf_f_using_rff} the norm of ${\boldf \in \RKHS}$ can be written as
\begin{equation}
    \| \boldsymbol{f} \|_{\mathcal{H}_{K}}^{2} = \| \boldalpha \|^{2}
\end{equation}
The vector-valued regularized least-squares problem in \eqref{eq:vector_valued_regular_least_squares} is then re-formulated as an optimization problem
over ${\boldalpha \in \Rd}$
\begin{equation}\label{eq:rff_vector_valued_regular_least_squares}
    \min_{\boldalpha \in \Rd} \frac{1}{N} \sum_{i=1}^{N} \| \boldPsi(\boldx_i)^{\T} \boldalpha - \boldsymbol{y}_{i} \|^{2} + \lambda \boldalpha^{\T} \boldalpha
\end{equation}
By defining
\begin{equation}
    \boldPhi = \bb \boldPsi(\boldx_1)^{\T} \\ \vdots \\ \boldPsi(\boldx_N)^{\T} \eb \in \R^{mN \times d}
    \; , \qquad
    \boldY = \bb \boldy_1 \\ \vdots \\ \boldy_N \eb \in \R^{mN}
\end{equation}
the optimization problem in \eqref{eq:rff_vector_valued_regular_least_squares} can be written as
\begin{equation}\label{eq:rff_vector_valued_regular_least_squares_2}
    \min_{\boldalpha \in \Rd} \frac{1}{N} \left( \boldPhi \boldalpha - \boldY \right)^{\T} \left( \boldPhi \boldalpha - \boldY \right) + \lambda \boldalpha^{\T} \boldalpha
\end{equation}
where the minimum is found when the gradient with respect to ${\boldalpha}$ is zero
\begin{equation}\label{eq:rff_vector_valued_regular_least_squares_minimum}
    \boldalpha^* = \inv{\left( \boldPhi^{\T} \boldPhi + \lambda N \eye \right)} \boldPhi^{\T} \boldY
\end{equation}
and the function value of the optimal vector field is
\begin{equation}\label{eq:rff_vector_valued_regular_least_squares_f_function}
    \boldf^{*}(\boldx) = \boldPsi(\boldx)^{\T} \boldalpha^*
\end{equation}


